Consensus of state of the art mortality prediction models: From all-cause mortality to sudden death prediction

Worldwide, many millions of people die suddenly and unexpectedly each year, either with or without a prior history of cardiovascular disease. Such events are sparse (once in a lifetime), many victims will not have had prior investigations for cardiac disease and many different definitions of sudden death exist. Accordingly, sudden death is hard to predict. This analysis used NHS Electronic Health Records (EHRs) for people aged $\geq$50 years living in the Greater Glasgow and Clyde (GG\&C) region in 2010 (n = 380,000) to try to overcome these challenges. We investigated whether medical history, blood tests, prescription of medicines, and hospitalisations might, in combination, predict a heightened risk of sudden death. We compared the performance of models trained to predict either sudden death or all-cause mortality. We built six models for each outcome of interest: three taken from state-of-the-art research (BEHRT, Deepr and Deep Patient), and three of our own creation. We trained these using two different data representations: a language-based representation, and a sparse temporal matrix. We used global interpretability to understand the most important features of each model, and compare how much agreement there was amongst models using Rank Biased Overlap. It is challenging to account for correlated variables without increasing the complexity of the interpretability technique. We overcame this by clustering features into groups and comparing the most important groups for each model. We found the agreement between models to be much higher when accounting for correlated variables. Our analysis emphasises the challenge of predicting sudden death and emphasises the need for better understanding and interpretation of machine learning models applied to healthcare applications.

==> supplimentary_material.tex <==

\title{Supplementary Material}

%\keywords{Keyword1, Keyword2, Keyword3}

\begin{document}

\section*{Appendix A: Text Vectorization Methods}
Two possible text vectorization methods are integer encoding and bag-of-words encoding. Both vectorization methods require a 'vocabulary', a set of unique words which could appear in the input text. The vocabulary used depends on the application; for a model translating French into English, this will be a set of French and English words. For healthcare applications, this can be ICD-10 codes and medications. Each vocabulary usually also contains an "unknown" token (which we refer to as [UNK], to account for words that are given to the model but do not appear in the vocabulary).

The bag-of-words encoding turns the language representation into a sparse vector, with each ‘feature’ in this representation being an event of interest. In contrast, in integer encoding each ‘feature’ in this representation is a sentence position. This is important when we consider interpretability. When considering global interpretability, we attempt to understand what features matter in the model. We do this by manipulating the values at each feature in the training or testing set. In integer encoding, this will give us the position in the sentence that matters most. For bag-of-words encoding, this gives us the words in the sentence that matter most, which we typically care about more than positional importance. Therefore, an extra step is required for integer encoding in order to generate event importance indices.

In integer encoding, each word in the vocabulary is assigned to a unique integer. We replace each word in the input sentence with its corresponding integer representation, creating a vector of integers for each sentence. In contrast, for bag-of-words representation, sentences are represented as how many times each word in the vocabulary appears in the sentence.

\section*{Appendix B: Interpretability Techniques}
In the following section we describe the two interpretability techniques used in this paper.

\subsection*{Permutation Feature Importance}
Permutation Feature Importance (PFI) is a method of global interpretability. It measures the difference in model performance after features are perturbed (Algorithm \ref{algorithm:pfi}) \cite{RN278}. If a feature is permuted and the model performance does not change, the feature was clearly unimportant to model decision making. Conversely, if a feature has a large impact on model performance, that feature contributed heavily to model decision making, and therefore the feature is important to the model.

\begin{algorithm}
    \begin{algorithmic}[1]
        \State Calculate original model error $e_{orig}$ using dataset $X$
        \For{each feature $j \in \{1,..,p\}$}
            \State Permute the feature $j$ in dataset $X$ to create a new dataset $X_{perm}$
            \State Calculate model error $e_{perm}$ based on new dataset $X_{perm}$
            \State Calculate feature importance $FI_j = e_{orig} - e_{perm}$
        \EndFor
        \State Sort feature importances $FI$ from most to least important
    \end{algorithmic}
\caption{Permutation Feature Importance Algorithm}
\label{algorithm:pfi}
\end{algorithm}

PFI is a very simple but very powerful tool, as it is easy to implement, easy to rationalise, model agnostic, and provides global interpretability. However, since each feature is permuted individually, it can produce unrealistic scenarios if features are highly correlated, which can affect the validity of global explanations.

\subsection*{LIME}
Local interpretable model-agnostic explanations (LIME) is a technique for generating local interpretations which explain what features a model is interested in when looking at a particular patient \cite{RN260}. It does this by perturbing each of the features in the patient record, passing the modified data back through the original model, then training an intrinsically interpretable model to mimic the behaviour of the more complex model, and interpreting the simpler model. The explanations produced by LIME can be described by the following equation:

\begin{equation}
    \upxi(x) = \underset{g \in G}{argmin}  \mathcal{L}(f,g,\pi_x) + \Omega(g)
\end{equation}

where:
\begin{itemize}
    \item $G$ is a class of interpretable models (e.g. a linear model or decision tree)
    \item $g$ is an intrinsically interpretable model from class $G$
    \item $\Omega(g)$ is a measure of the complexity of the explanation $g \in G$
    \item $f$ is the original "complex" model
    \item $\pi_x$ is a locality measure, how large a neighborhood we consider around datapoint $x$
    \item $\mathcal{L}$ is a fidelity function (how faithful the explanation is to the underlying model)
\end{itemize}

as defined in the original paper \cite{RN260}.

\section*{Appendix C: Outcome Definition}
In this study, we predict for both all-cause mortality and sudden death within 6 months of the index date, given the past year of patient medical records. For our outcome groups, this index date becomes a random date up to 6 months (between 0 and 180 days) before date of death. Our control group when predicting sudden death and other catastrophic cardiovascular events is a group of people in the SafeHaven dataset who are not already sick; this index date is a randomly selected date in which the individual did not suffer a catastrophic cardiovascular event within the following six months.

A flow diagram of how we define our sudden death and other catastrophic cardiovascular event population can be found in Figure \ref{fig:pop_def}.

\begin{figure}[ht]
\centering
\includegraphics[width=0.7\textwidth]{figures/population_definition.png}
\caption{Population Definition Flow Diagram. This figure gives a flow diagram of how we convert a control and event group to a training and testing set which can be used by our machine learning models.}
\label{fig:pop_def}
\end{figure}

\section*{Appendix D: Feature Processing}
In the following section, we describe how we create both our language model and sparse matrix data representations from individual feature tables within the NHS Safe Haven dataset.

\subsection*{Feature Processing}
\begin{itemize}
    \item \textbf{Prescriptions} In our dataset, prescriptions are represented as BNF codes; we represent each medication as the first four digits of the BNF code.
    \item \textbf{Hospitalisations} In our dataset, hospital records contain up to six diagnoses for each visit, with each diagnosis given as an ICD-10 code. We take the first two diagnoses (primary and secondary diagnosis for each visit) and represent each diagnosis as the first four digits of the ICD-10 code.
    \item \textbf{Blood tests} The blood test dataset is the noisiest dataset we work with in this study, and therefore requires the most pre-processing. We group blood tests into 42 unique categories (41 blood test types, e.g. haemoglobin, calcium, etc, plus 'other'). We capture six types of information from the blood test dataset:
    \begin{itemize}
        \item A marker that a test was taken (e.g. calcium was tested)
        \item The result of each test (numerical, e.g. 2.2 mmol/L)
        \item How many samples of blood were taken in hospital for each patient (secondary care)
        \item How many samples of blood were taken by a GP for each patient (primary care)
        \item We then group our 41 variables into eight blood test families: full blood count, diabetes, renal, bone and liver, thyroid, cholesterol, inflammation, and coagulation. We record how many tests of each group were taken in hospital (primary care) and in hospital (secondary care)
    \end{itemize}
    For the results of each test, we filter out clinically impossible blood tests (e.g. a red blood cell count of zero), and label these values as 'missing'. For the rest of the categories, we include a simple count of how many of each test was taken.
    \item \textbf{Demographics} We record the age and sex at index date for each patient
    \item \textbf{History of major disease} For each patient, we focus on 11 of the following major diseases, and define this as being hospitalised for each disease at any point in the person's history:
    \begin{itemize}
        \item Heart failure
        \item Chronic ischemic heart disease
        \item Liver disease
        \item Seizures
        \item Stroke
        \item Kidney disease
        \item Primary hypertension
        \item Hypertensive heart disease
        \item Chronic kidney disease
        \item Type 1 diabetes
        \item Type 2 diabetes
    \end{itemize}
\end{itemize}

\subsection*{Language Model}

In language models, healthcare records are encoded as sentences which are broken down in to keywords allowing key medical concepts and time-dependent information to be represented. For each hospital diagnosis, medication prescription, and blood test, each code is pre-pended with a feature type identifier ($h\_$, $m\_$ and $t\_$ respectively). Each feature is binned into 2 month intervals, and events are sorted from most to least recent month (from index). Each new month is marked by a $segment\_x$ feature, where x is the number of months working backwards from index. For example, [$segment\_0$ $h\_I50$ $segment\_1$ $m\_0202$] tells us a hospital diagnosis of code I50 (heart failure) was given at the most recent month, with a prescription of code 0202 (diuretics) was given the month previously. We add 2 additional features to the end of each sentence, a feature giving the person's sex, and a feature giving the person's age at index. We then add any history of major disease at the end of each sentence, with each condition prepended by a $hist\_$ identifier. An example of this can be seen in Figure \ref{fig:sentence}.

\begin{figure}[ht]
\centering
\includegraphics[width=0.5\textwidth]{figures/sentence.png}
\caption{Encoded Sentence Example. This figure gives an example sentence which is used to represent patient records. The sentence is split into 'segments' (month 0, 1, 2, 3 and 4). Colours have been used to highlight different types of features; red indicates time, green indicates events, and blue indicates 'static' variables such as age and sex.}
\label{fig:sentence}
\end{figure}

\subsection*{Sparse Temporal Matrix}
We encode all hospitalisations, medications and blood tests into their distinct categories as discussed previously. Each event is then binned into 2 month chunks, totalling 7 possible chunks between $index$ and $index - 1   year$. We then create a 2D matrix for each patient, of size $n\_features \times n\_time\_windows$. Each patients history is then added to the appropriate cell, where a value of 1 at feature $f$ and time $t$ indicates that an event of type f occurred t months before index. Finally, we add 13 constant features: two demographic columns (age and sex) and 11 variables indicating history of major disease, where each of these features are duplicated for all discrete time intervals. The result is a sparse 2D matrix for each patient which gives a marker of when different types of events occurred in the year before index, plus age and sex. The final array is a 3D matrix of size $n\_patients \times n\_features \times n\_time\_windows$.  The array for all patients is stored in $(i,j,k,v)$ form, where $i$ is the patient, $j$ is the feature, $k$ is the time, and $v$ is the value at that cell. The size of the final matrix is also saved, meaning the dataset can be rebuilt before being passed into each model.

\section*{Appendix E: Model Construction Details}
In this section, we describe implementation details of each of the five models under test in this study.

\begin{itemize}
    \item \textbf{\textit{BEHRT}} As discussed, we train BEHRT by first passing it the entire patient dataset with unsupervised learning, trained using a masked language model. The model is then fine tuned for the prediction of sudden death and other catastrophic cardiovascular events. As with the original BEHRT model, the first layer is a TextVectorizer with integer encoding, fed into a feedforward multi-headed self-attention network, with four layers consisting of 20 heads in each, and an embedding layer of size 256.
    \item \textbf{\textit{Deepr}} Like BEHRT, the first layer of this model is a TextVectorizer with integer encoding. This is fed into a 1D convolutional layer with 45 filters, which is then passed into a max pooling layer, then finally a dense layer for the prediction of the outcome of interest. Like in \cite{RN262} we add a second model input to give the model demographic information (specifically age and sex), via an extra dense layer.
    \item \textbf{\textit{DeepPatient}} For DeepPatient, we use a 3-layer stack of denoising autoencoders for model pre-training using unsupervised learning. The model is trained to reconstruct the original training data which has been corrupted by randomly setting a proportion of the input data to zero (in this case we use 5\%). For the denoising autoencoder, we use 3x 500 neuron fully connected layers as an encoder, followed by a stack of 3x 500 neuron fully connected layers as a decoder. Once the autoencoder has been trained, the decoder is chopped off and the output of the encoder is fed to a downstream classification model (in this case, a GRU).
    \item \textbf{\textit{GRU (language)}} For the language GRU, we use the TextVectorizer as with both BEHRT and Deepr models. Unlike these models, we use a bag-of-words count based encoding to create a sparse vector of size \textit{vocab\_size} for each patient. Our GRU consists of 5 layers; a 100-unit layer and a 50-unit layer with a dropout layer of 10\% and 30\% after each layer respectively. The final dropout layer is fed into a fully connected layer with 2 input neurons.
    \item \textbf{\textit{GRU (sparse)}} The sparse representation of both our GRU is very similar to our language model representation, with the same architecture for both. However, because our sparse matrix is already in machine readable form. we do not need to pass it through a vectorize layer.
\end{itemize}

\section*{Appendix F: Statistical Comparison Techniques}
\subsection*{Ranked Biased Overlap}
Rank Biased Overlap (RBO) is an alternative to Kendall Tau correlation for calculating the similarity between two ranked lists. Unlike Kendall-Tau, it weights the head of the list as more important than the tail (the weighting of which is defined by tuneable parameter P). This is especially important in our case, as many of the features in our lists have the same feature importance (zero), and are therefore ordered randomly. RBO is defined as the following equation \cite{RN275}:\\

$$
\mathrm{RBO}(\mathrm{S}, \mathrm{T}, \mathrm{p}, \mathrm{k})=\frac{\mathrm{X}_{\mathrm{k}}}{\mathrm{k}} \cdot \mathrm{p}^{\mathrm{k}}+\frac{1-\mathrm{p}}{\mathrm{p}} \sum_{\mathrm{d}=1}^{\mathrm{k}} \frac{\mathrm{X}_{\mathrm{d}}}{\mathrm{d}} \cdot \mathrm{p}^{\mathrm{d}}
$$\\

where:\\
\begin{itemize}
    \item S and T are two ranked lists under test
    \item d is the depth being examined
    \item k is the max depth of the list
    \item $X_a$ is the size of the overlap between S adn T up to depth a
    \item p is a tuneable parameter which tells the function how much weight to put at the head of the list compared to the tail
\end{itemize}

\section*{Appendix G: Final Feature List}

\begin{itemize}
    \item 318 hospitalisation variables
    \item 196 medication variables
    \item 103 blood test variables
    \item 10 variables indicating history of major disease
    \item 2 demographic variables (age and sex)
\end{itemize}

\section*{Appendix H: Training Curves}
\begin{figure}[h!]
\centering
\includegraphics[scale=0.5]{figures/deeppatient/pretraining.png}
\caption{DeepPatient Pre-Training Plot. This figure gives the training curves for the pre-training step of the DeepPatient model. Training accuracy is given in blue, validation accuracy is given in orange.}
\label{fig:deeppatient_pretraining}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[scale=0.5]{figures/behrt/pretraining.png}
\caption{BEHRT Pre-Training Plot. This figure gives the training curves for the pre-training step of the BEHRT model.}
\label{fig:behrt_pretraining}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{figures/deeppatient/training.png}
\includegraphics[width=0.45\textwidth]{figures/deeppatient/training_raw.png}
\caption{Deep Patient Training Curves. This graph gives the training and validation curves for the Deep Patient model trained for 10 epochs. The first plot gives the scale between 0.0 and 1.0, the second plot gives the scale auto-adjusted so we can see how the model trains over time}
\label{fig:deeppatient_training}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{figures/deepr/training.png}
\includegraphics[width=0.45\textwidth]{figures/deepr/training_raw.png}
\caption{Deepr Training Curves. This graph gives the training and validation curves for the Deepr model trained for 10 epochs. The first plot gives the scale between 0.0 and 1.0, the second plot gives the scale auto-adjusted so we can see how the model trains over time.}
\label{fig:deepr_training}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{figures/language_gru/training.png}
\includegraphics[width=0.45\textwidth]{figures/language_gru/training_raw.png}
\caption{Language GRU Training Curves. This graph gives the training and validation curves for the language GRU model trained for 10 epochs. The first plot gives the scale between 0.0 and 1.0, the second plot gives the scale auto-adjusted so we can see how the model trains over time}
\label{fig:language_gru_training}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{figures/sparse_gru/training.png}
\includegraphics[width=0.45\textwidth]{figures/sparse_gru/training_raw.png}
\caption{Sparse GRU Training Curves. This graph gives the training and validation curves for the sparse GRU model trained for 10 epochs. The first plot gives the scale between 0.0 and 1.0, the second plot gives the scale auto-adjusted so we can see how the model trains over time}
\label{fig:sparse_gru_training}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.45\textwidth]{figures/behrt/training.png}
\includegraphics[width=0.45\textwidth]{figures/behrt/training_raw.png}
\caption{BEHRT Training Curves. This graph gives the training and validation curves for the BEHRT model trained for 10 epochs. The first plot gives the scale between 0.0 and 1.0, the second plot gives the scale auto-adjusted so we can see how the model trains over time}
\label{fig:behrt_training}
\end{figure}

\clearpage

\section*{Appendix I: Clustering Details}
\subsection*{Spectral Co-Clustering Equation}
Spectral co-clustering is defined by the following two equations \cite{coclustering_original}:

\begin{equation}
\mathcal{W}_m=\left\{w_i: \sum_{j \in \mathcal{D}_m} A_{i j} \geq \sum_{j \in \mathcal{D}_t} A_{i j}, \forall l=1, \ldots, k\right\}\\
\mathcal{D}_m=\left\{d_j: \sum_{i \in \mathcal{W}_m} A_{i j} \geq \sum_{i \in \mathcal{W}_l} A_{i j}, \forall l=1, \ldots, k\right\}
\end{equation}

where:
\begin{itemize}
    \item $A$ is the matrix to be clustered
    \item $W$ and $D$ are the interconnected sets of clusters in two dimensions
\end{itemize}

Since these two equations depend on each other, these two processes are recursively applied to $A$ until a stable optimum is reached.

\subsection*{Optimum Number of Clusters using the Elbow Method}
\begin{figure}[h]
\centering
\includegraphics[width=\textwidth]{figures/finding_optimum_clusters.png}
\caption{Finding Optimum Number of Clusters \textmd{The top plot shows a plot of the number of single-feature clusters as the number of clusters increases. The bottom plot shows the sum of squared distances between each feature and the centroid of its clusters, obtained using the Elbow method. Both of these plots are used to determine the optimum number of clusters for this analysis.}}
\label{fig:biclustering_optimum}
\end{figure}

\clearpage

\bibliography{state_of_the_art_references}
\bibliographystyle{ieeetr}

\end{document}

\section*{Appendix J: Calibration Curves}
We give the calibration curves for each of our five models plus our baseline model when predicting sudden death and other catastrophic cardiovascular events versus all-cause mortality in Figures \ref{fig:calibration_curves_deeppatient}, \ref{fig:calibration_curves_deepr}, \ref{fig:calibration_curves_language_gru}, \ref{fig:calibration_curves_sparse_gru}, and \ref{fig:calibration_curves_behrt}. From these figures, it appears that BEHRT has the best calibration of the six, with Deep Patient having the worst calibration across both outcomes, while also having the lowest AUC of the five models, shown in Table \ref{table:machine_learning_results}. It is clear that all of our models favour lower probabilities, likely the effect of the uneven class distribution in our data.

\begin{figure}[h!]
\centering
\includegraphics[width=0.6\textwidth]{figures/calibration_deep_patient.png}
\caption{Model Calibration Curves \textmd{This graph gives the calibration curves for our Deep Patient model. The 'ideal' calibration can be seen in orange, the actual calibration is given in blue.}}
\label{fig:calibration_curves_deeppatient}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.6\textwidth]{figures/calibration_deepr.png}
\caption{Model Calibration Curves \textmd{This graph gives the calibration curves for our Deepr model. The 'ideal' calibration can be seen in orange, the actual calibration is given in blue.}}
\label{fig:calibration_curves_deepr}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.6\textwidth]{figures/calibration_language_gru.png}
\caption{Model Calibration Curves \textmd{This graph gives the calibration curves for our language GRU model. The 'ideal' calibration can be seen in orange, the actual calibration is given in blue.}}
\label{fig:calibration_curves_language_gru}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.6\textwidth]{figures/calibration_sparse_gru.png}
\caption{Model Calibration Curves \textmd{This graph gives the calibration curves for our sparse GRU model. The 'ideal' calibration can be seen in orange, the actual calibration is given in blue.}}
\label{fig:calibration_curves_sparse_gru}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=0.6\textwidth]{figures/calibration_behrt.png}
\caption{Model Calibration Curves \textmd{This graph gives the calibration curves for our BEHRT model. The 'ideal' calibration can be seen in orange, the actual calibration is given in blue.}}
\label{fig:calibration_curves_behrt}
\end{figure}

